An Asymptotic Preserving Scheme for the Euler equations in a strong magnetic field

This paper is concerned with the numerical approximation of the isothermal Euler equations for charged particles subject to the Lorentz force. When the magnetic field is large, the so-called drift-fluid approximation is obtained. In this limit, the parallel motion relative to the magnetic field direction splits from perpendicular motion and is given implicitly by the constraint of zero total force along the magnetic field lines. In this paper, we provide a well-posed elliptic equation for the parallel velocity which in turn allows us to construct an Asymptotic-Preserving (AP) scheme for the Euler-Lorentz system. This scheme gives rise to both a consistent approximation of the Euler-Lorentz model when epsilon is finite and a consistent approximation of the drift limit when epsilon tends to 0. Above all, it does not require any constraint on the space and time steps related to the small value of epsilon. Numerical results are presented, which confirm the AP character of the scheme and its Asymptotic Stability.

==> palette.tex <==
\def\filename{palette.tex}
\def\fileversion{0.91}
\def\filedate{92/09/02}
%
% Send comments to the author: Fred Knight (knight@ll.mit.edu)
% 
% Purpose:
%   Macros to get colors from a palette.
%   For use with PSTricks version v0.91 and later.
%   These macros allow the user to select colors from a palette derived
%   from the Openwindows file rgbcolors.txt, which contains about 140 
%   distinct colors, not including different shades and gray levels.
%   The user can also display the palette and add to it.
% Usage:
%   \palette
%      the list of colors and values, only an internal list of colors
%   \addtopalette[type]{name}{values}
%      add a color to \palette
%      type---an integer denoting the type of values
%         1 = rgb, default, 3 numbers between 0 (low) and 1 (high)
%         2 = hsb, 3 numbers between 0 (low) and 1 (high)
%         3 = cmyk, 4 numbers between 0 (low) and 1 (high)
%         4 = gray, 1 number between 0 (low) and 1 (high)
%      name---the color's name as stored in \palette,
%         usually all lowercase
%      values---numbers according to the type of color
%      Examples:
%         \addtopalette{mud}{0.6 0.4 0.2}
%         \addtopalette[4]{mudgray}{0.4}
%   \addrgb{name}{values}
%      add an rgb color called name to the palette
%   \addhsb{name}{values}
%      add an hsb color called name to the palette
%   \addcmyk{name}{values}
%      add an cmyk color called name to the palette
%   \addgray{name}{values}
%      add an gray color called name to the palette
%   \getcolor[altname]{name}
%      analogous to \newrgbcolor but get values from
%      \palette and define a macro \name or \altname, if present.
%      Examples:
%         \getcolor{thistle} {\thistle The color is slightly off purple.}
%         \getcolor[goo]{brown} {\goo Its fragrance graced the table.}
%   \showpalette
%      macro to show all the colors in \palette
% Restrictions:
%   Works only with PostScript and requires PSTricks.
% Acknowledgement:
%   Thanks to Tim Van Zandt for many helpful comments.
% 
%
% =====>> Preliminaries: Is PSTricks loaded?  Change catcode of @.
%
\ifx\pstricksloaded\relax\else\input pstricks\fi
\typeout{`\filename' v\fileversion\space\space <\filedate> (Fred Knight)}
\edef\theatcode{\the\catcode`\@}
\ifnum\theatcode=13\let\theat @\fi
\catcode`\@=11\relax
%
% =====>> User macros for adding colors to \palette: 4 types
%
\def\addtopalette{\@ifnextchar [{\@addtopalette}{\@addtopalette[1]}}
\def\@addtopalette[#1]#2#3{\edef\palette{\palette(#2,#1,#3)}}
\def\addrgb{\addtopalette[1]}
\def\addhsb{\addtopalette[2]}
\def\addcmyk{\addtopalette[3]}
\def\addgray{\addtopalette[4]}
%
% =====>> User macro to define a new color name.
%
\def\getcolor{\@ifnextchar [{\@getcolor}{\@getcolor[\@nil]}}
\def\@getcolor[#1]#2{%
  \ifx#1\@nil\def\altname{#2}\else\def\altname{#1}\fi
  \def\pst@tempg##1(#2,##2,##3)##4\@nil{%
    \ifcase##2\@pstrickserr{Color `#2' not found}\@eha
    \or\newrgbcolor{\altname}{##3}%
    \or\newhsbcolor{\altname}{##3}%
    \or\newcmykcolor{\altname}{##3}%
    \or\newgray{\altname}{##3}%
    \fi}%
  \expandafter\pst@tempg\palette(#2,0,)\@nil}
%
% =====>> \showpalette and its parts.
%
% Define 4 dimensions for \showpalette
\newdimen\PalBoxwd\PalBoxwd=\hsize
\newdimen\PalBoxht\PalBoxht=\baselineskip
\newdimen\savedparindent
\newdimen\savedparskip
% Each color gets a rule with text of two colors (black & white) in it.
\def\paletteBox{\vrule height\PalBoxht width\PalBoxwd depth1ex}
% Each color has 2 entries: one with black text, the other with white.
\def\paletteEntry#1#2#3{%
  \hbox to 0.5\hsize{ #1\hss
  \ifcase#2\or rgb\or hsb\or cmyk\or gray\fi:#3 }}
\def\showpalette{\edef\pst@tempa{\palette(NoMoreColors,0, 0)}%
  \savedparskip=\parskip\parskip0pt
  \savedparindent=\parindent\parindent0pt\par
  \expandafter\thepalette\pst@tempa
  \parindent=\savedparindent
  \parskip=\savedparskip}
% \thepalette loops through the entries of \palette.
\def\thepalette(#1,#2,#3){%
  \ifnum#2=0
    \let\next\relax
  \else
    \leavevmode
    \hbox{%
      \pstVerb{#3 \ifcase#2\or setrgbcolor\or sethsbcolor\or
        setcmykcolor\or setgray\fi}%
      \paletteBox\hskip-\hsize
      \pstVerb{0 setgray}\paletteEntry{#1}{#2}{#3}% black text
      \pstVerb{1 setgray}\paletteEntry{#1}{#2}{#3}}% white text
    \let\next\thepalette
    \par\vskip1pt
  \fi\next}
%
% =====>> The palette of colors; derived from OPENWINDOWS/rgbcolors.txt.
%
\def\palette{%
% format: (name,type, values)
% where
%   name = name of the color
%   type = 1 for rgb, 2 for hsb, 3 for cmyk, 4 for gray
%   values = color values in the type specified
  (snow,1,1.00 0.98 0.98)% The color snow has r=1.00, b=0.98, and g=0.98.
  (ghostwhite,1,0.97 0.97 1.00)%
  (whitesmoke,1,0.96 0.96 0.96)%
  (gainsboro,1,0.86 0.86 0.86)%
  (floralwhite,1,1.00 0.98 0.94)%
  (oldlace,1,0.99 0.96 0.90)%
  (linen,1,0.98 0.94 0.90)%
  (antiquewhite,1,0.98 0.92 0.84)%
  (papayawhip,1,1.00 0.94 0.84)%
  (blanchedalmond,1,1.00 0.92 0.80)%
  (bisque,1,1.00 0.89 0.77)%
  (peachpuff,1,1.00 0.85 0.73)%
  (navajowhite,1,1.00 0.87 0.68)%
  (moccasin,1,1.00 0.89 0.71)%
  (cornsilk,1,1.00 0.97 0.86)%
  (ivory,1,1.00 1.00 0.94)%
  (lemonchiffon,1,1.00 0.98 0.80)%
  (seashell,1,1.00 0.96 0.93)%
  (honeydew,1,0.94 1.00 0.94)%
  (mintcream,1,0.96 1.00 0.98)%
  (azure,1,0.94 1.00 1.00)%
  (aliceblue,1,0.94 0.97 1.00)%
  (lavender,1,0.90 0.90 0.98)%
  (lavenderblush,1,1.00 0.94 0.96)%
  (mistyrose,1,1.00 0.89 0.88)%
  (white,1,1.00 1.00 1.00)%
  (black,1,0.00 0.00 0.00)%
  (midnightblue,1,0.10 0.10 0.44)%
  (navy,1,0.00 0.00 0.50)%
  (navyblue,1,0.00 0.00 0.50)%
  (cornflowerblue,1,0.39 0.58 0.93)%
  (darkslateblue,1,0.28 0.24 0.55)%
  (slateblue,1,0.42 0.35 0.80)%
  (mediumslateblue,1,0.48 0.41 0.93)%
  (lightslateblue,1,0.52 0.44 1.00)%
  (mediumblue,1,0.00 0.00 0.80)%
  (royalblue,1,0.25 0.41 0.88)%
  (blue,1,0.00 0.00 1.00)%
  (dodgerblue,1,0.12 0.56 1.00)%
  (deepskyblue,1,0.00 0.75 1.00)%
  (skyblue,1,0.53 0.81 0.92)%
  (lightskyblue,1,0.53 0.81 0.98)%
  (steelblue,1,0.27 0.51 0.71)%
  (lightsteelblue,1,0.69 0.77 0.87)%
  (lightblue,1,0.68 0.85 0.90)%
  (powderblue,1,0.69 0.88 0.90)%
  (paleturquoise,1,0.69 0.93 0.93)%
  (darkturquoise,1,0.00 0.81 0.82)%
  (mediumturquoise,1,0.28 0.82 0.80)%
  (turquoise,1,0.25 0.88 0.82)%
  (cyan,1,0.00 1.00 1.00)%
  (lightcyan,1,0.88 1.00 1.00)%
  (cadetblue,1,0.37 0.62 0.63)%
  (mediumaquamarine,1,0.40 0.80 0.67)%
  (aquamarine,1,0.50 1.00 0.83)%
  (darkgreen,1,0.00 0.39 0.00)%
  (darkolivegreen,1,0.33 0.42 0.18)%
  (darkseagreen,1,0.56 0.74 0.56)%
  (seagreen,1,0.18 0.55 0.34)%
  (mediumseagreen,1,0.24 0.70 0.44)%
  (lightseagreen,1,0.13 0.70 0.67)%
  (palegreen,1,0.60 0.98 0.60)%
  (springgreen,1,0.00 1.00 0.50)%
  (lawngreen,1,0.49 0.99 0.00)%
  (green,1,0.00 1.00 0.00)%
  (chartreuse,1,0.50 1.00 0.00)%
  (mediumspringgreen,1,0.00 0.98 0.60)%
  (greenyellow,1,0.68 1.00 0.18)%
  (limegreen,1,0.20 0.80 0.20)%
  (yellowgreen,1,0.60 0.80 0.20)%
  (forestgreen,1,0.13 0.55 0.13)%
  (olivedrab,1,0.42 0.56 0.14)%
  (darkkhaki,1,0.74 0.72 0.42)%
  (khaki,1,0.94 0.90 0.55)%
  (palegoldenrod,1,0.93 0.91 0.67)%
  (lightgoldenrodyellow,1,0.98 0.98 0.82)%
  (lightyellow,1,1.00 1.00 0.88)%
  (yellow,1,1.00 1.00 0.00)%
  (gold,1,1.00 0.84 0.00)%
  (lightgoldenrod,1,0.93 0.87 0.51)%
  (goldenrod,1,0.85 0.65 0.13)%
  (darkgoldenrod,1,0.72 0.53 0.04)%
  (rosybrown,1,0.74 0.56 0.56)%
  (indianred,1,0.80 0.36 0.36)%
  (saddlebrown,1,0.55 0.27 0.07)%
  (sienna,1,0.63 0.32 0.18)%
  (peru,1,0.80 0.52 0.25)%
  (burlywood,1,0.87 0.72 0.53)%
  (beige,1,0.96 0.96 0.86)%
  (wheat,1,0.96 0.87 0.70)%
  (sandybrown,1,0.96 0.64 0.38)%
  (tan,1,0.82 0.71 0.55)%
  (chocolate,1,0.82 0.41 0.12)%
  (firebrick,1,0.70 0.13 0.13)%
  (brown,1,0.65 0.16 0.16)%
  (darksalmon,1,0.91 0.59 0.48)%
  (salmon,1,0.98 0.50 0.45)%
  (lightsalmon,1,1.00 0.63 0.48)%
  (orange,1,1.00 0.65 0.00)%
  (darkorange,1,1.00 0.55 0.00)%
  (coral,1,1.00 0.50 0.31)%
  (lightcoral,1,0.94 0.50 0.50)%
  (tomato,1,1.00 0.39 0.28)%
  (orangered,1,1.00 0.27 0.00)%
  (red,1,1.00 0.00 0.00)%
  (hotpink,1,1.00 0.41 0.71)%
  (deeppink,1,1.00 0.08 0.58)%
  (pink,1,1.00 0.75 0.80)%
  (lightpink,1,1.00 0.71 0.76)%
  (palevioletred,1,0.86 0.44 0.58)%
  (maroon,1,0.69 0.19 0.38)%
  (mediumvioletred,1,0.78 0.08 0.52)%
  (violetred,1,0.82 0.13 0.56)%
  (magenta,1,1.00 0.00 1.00)%
  (violet,1,0.93 0.51 0.93)%
  (plum,1,0.87 0.63 0.87)%
  (orchid,1,0.85 0.44 0.84)%
  (mediumorchid,1,0.73 0.33 0.83)%
  (darkorchid,1,0.60 0.20 0.80)%
  (darkviolet,1,0.58 0.00 0.83)%
  (blueviolet,1,0.54 0.17 0.89)%
  (purple,1,0.63 0.13 0.94)%
  (mediumpurple,1,0.58 0.44 0.86)%
  (thistle,1,0.85 0.75 0.85)%
}
\expandafter\catcode`\@=\theatcode\relax
\ifnum\theatcode=13\let @\theat\fi
\endinput

